Access Trends of In-network Cache for Scientific Data

Scientific collaborations are increasingly relying on large volumes of data for their work and many of them employ tiered systems to replicate the data to their worldwide user communities. Each user in the community often selects a different subset of data for their analysis tasks; however, members of a research group often are working on related research topics that require similar data objects. Thus, there is a significant amount of data sharing possible. In this work, we study the access traces of a federated storage cache known as the Southern California Petabyte Scale Cache. By studying the access patterns and potential for network traffic reduction by this caching system, we aim to explore the predictability of the cache uses and the potential for a more general in-network data caching. Our study shows that this distributed storage cache is able to reduce the network traffic volume by a factor of 2.35 during a part of the study period. We further show that machine learning models could predict cache utilization with an accuracy of 0.88. This demonstrates that such cache usage is predictable, which could be useful for managing complex networking resources such as in-network caching.

==> Makefile <==
###############################################################################
# the latex command is pdflatex
LATEX = pdflatex -shell-escape
# the bibtex command is biber -- specified in preamble.tex in this directory
BIBTEX = bibtex

###############################################################################
# the main latex file 
MAIN = main

###############################################################################
# Assume all LaTeX files (*.tex) are in this level and all figures are in figs
# directory and all bibtex entries are at this level with .bib
TEXFILES = ${wildcard *.tex} ${wildcard */*.tex}
BIBFILES = ${wildcard *.bib}
FIGS = ${figs/wildcard *.pdf} ${figs/wildcard *.png} ${figs/wildcard *.jpg}

###############################################################################
# default target
.DEFAULT_GOAL := $(MAIN).pdf
$(MAIN): $(MAIN).pdf
.PHONY: $(MAIN) clean realclean

###############################################################################
# run LATEX command to generate the main PDF file
$(MAIN).pdf $(MAIN).log: $(TEXFILES) $(FIGS) $(BIBFILES)
	${LATEX} $(MAIN)
	@if [ `fgrep undefined $(MAIN).log | fgrep Citation - | wc -l` -gt 0 ]; then \
	${BIBTEX} $(MAIN); ${LATEX} $(MAIN); fi;
	@if [ `fgrep undefined $(MAIN).log | fgrep Citation - | wc -l` -gt 0 ]; then \
	${BIBTEX} $(MAIN); ${LATEX} $(MAIN); fi;
	@while [ `fgrep -i 'Rerun ' $(MAIN).log | fgrep LaTeX - | wc -l` -gt 0 ]; do \
        ${LATEX} $(MAIN); \
        done

###############################################################################
# basic sanity check
check: missingincludes badrefs badbibs

# Extract a list of missing smartinclude files
missingincludes: $(MAIN).log
	@(grep -i "smartinclude: warning:" $< | \
	  sed 's/smartinclude: WARNING: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== SMARTINCLUDE WARNINGS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

# Check log for: 
# - Multiply defined labels
# - Undefined labels
# - Undefined citations
# - Undefined acronyms (no messages for multiply-defined acronyms)
badrefs: $(MAIN).log
	@(grep -i "latex warning:" $< |\
	  grep -v -i "there were multiply-defined labels" | \
	  grep "multiply defined" |\
	  sed 's/LaTeX Warning: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MULTIPLY-DEFINED LABELS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "latex warning:" $< | \
	  grep -v -i "there were undefined references" | \
	  grep -i "reference" | grep -i "undefined" |\
	  sed 's/LaTeX Warning: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED LABELS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "package acronym warning:" $< | \
	  grep -i "acronym" | grep -i "not defined" |\
	  sed 's/Package acronym Warning: //' |\
	  sort | uniq > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED ACRONYMS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

# Check BibTeX log for:
# - missing .bib files
# - missing database entries
# - repeated entries
# - string name undefined
# - errors in entries ("I was expecting...")
badbibs: $(MAIN).log
	${BIBTEX} $(MAIN)
	@(grep -i "i couldn't open database file " $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MISSING BIB FILES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "warning--i didn't find a database entry for" \
	  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MISSING BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "repeated entry--"  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== REPEATED BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "warning--string name" $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED STRINGS IN BIB =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "i was expecting"  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== ERRORS IN BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

clean:
	-@find . \( -name '*.aux' -print \) -o \( -name '*.log' -print \) \
		-o \( -name '*.bbl' -print \) -o \( -name '*.blg' -print \) \
		-o \( -name '*.toc' -print \) -o \( -name '*.out' -print \) \
		-o \( -name '*.bcf' -print \) -o \( -name '*~' -print \) \
		-o \( -name '*.maf' -print \) -o \( -name '*.mtc*' -print \) | xargs $(RM)

###############################################################################
# WARNING: removes the main target
realclean: clean
	$(RM) $(MAIN).pdf*

